Data Roaming and Quality Assessment for Composed Image Retrieval

The task of Composed Image Retrieval (CoIR) involves queries that combine image and text modalities, allowing users to express their intent more effectively. However, current CoIR datasets are orders of magnitude smaller compared to other vision and language (V&L) datasets. Additionally, some of these datasets have noticeable issues, such as queries containing redundant modalities. To address these shortcomings, we introduce the Large Scale Composed Image Retrieval (LaSCo) dataset, a new CoIR dataset which is ten times larger than existing ones. Pre-training on our LaSCo, shows a noteworthy improvement in performance, even in zero-shot. Furthermore, we propose a new approach for analyzing CoIR datasets and methods, which detects modality redundancy or necessity, in queries. We also introduce a new CoIR baseline, the Cross-Attention driven Shift Encoder (CASE). This baseline allows for early fusion of modalities using a cross-attention module and employs an additional auxiliary task during training. Our experiments demonstrate that this new baseline outperforms the current state-of-the-art methods on established benchmarks like FashionIQ and CIRR.

==> tables/TTI_clip.tex <==
\begin{table}[ht]
\begin{center}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccccc|c}
\hline
Dataset & R@1 & R@5 & R@10 & R@50 & R@100 & \multicolumn{1}{l|}{R@500} & \multicolumn{1}{l}{\%CT2I} \\ \hline
COCO & 32.69 & 57.76 & 68.23 & 90.07 & 96.21 & 99.56 & 60.17 \\
CIRR & 19.97 & 44.61 & 57.07 & 80.12 & 86.70 & 97.03 & 48.23 \\
FashionIQ & 6.07 & 12.55 & 16.84 & 31.85 & 41.57 & 66.74 & 16.82 \\
LaSCo & \textbf{1.47} & \textbf{3.81} & \textbf{5.89} & \textbf{14.56} & \textbf{20.89} & \textbf{45.64} & \textbf{6.61} \\ \hline
\end{tabular}
}
\end{center}
\caption{Results of CLIP Text-to-Image (CT2I) baseline on several datasets. Retrieval on datasets that require compositional capabilities is expected to be low, since query-text is used. \%CT2I score is the average of R@\{1,10,50\}.}
\label{tab:tti_clip}
\end{table}

==> tables/amt.tex <==
\begin{table}[ht]
\begin{center}
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{@{}llll@{}}
\toprule
 & LaSCo & FashionIQ & CIRR \\ \midrule
MOS & 3.58 & 3.77& 3.91 \\
Positive Rate & 86.5\% & 92.9\% & 95.9\% \\
\bottomrule
\end{tabular}
}
\end{center}
\caption{User study}
\label{tab:amt_user_study}
\end{table}

==> tables/cirr_val.tex <==
\begin{table}[ht]
\begin{center}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cl|cccc|ccc}
\hline
\multicolumn{1}{l}{} &  & \multicolumn{4}{c|}{Recall@K} & \multicolumn{3}{c}{$\text{R}_{\text{subset}}$@K} \\
\multicolumn{1}{l}{Mode} & \our ver. & K=1 & K=5 & K=10 & K=50 & K=1 & K=2 & K=3 \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Zero\\ Shot\end{tabular}} & Init & 16.63 & 33.54 & 42.65 & 65.30 & 55.74 & 77.11 & 88.48 \\
 & Pre. LaSCo & 30.89 & 60.75 & 73.88 & 92.84 & 60.63 & 80.17 & 90.41 \\
 & Pre. LaSCo w/cap. & 35.40 & 65.78 & 78.53 & 94.63 & 64.29 & 82.66 & 91.61 \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Finetuned\\ on\\ CIRR\end{tabular}} & Text-only & 39.01 & 69.53 & 79.24 & 91.32 & 78.68 & 91.7 & 96.08 \\
 & Image-only & 0.0 & 0.19 & 0.41 & 2.12 & 19.78 & 39.49 & 59.87 \\
 & \our & 48.00 & 79.11 & 87.25 & \textbf{97.57} & 75.88 & \textbf{90.58} & \textbf{96.00} \\
 & Pre. LaSCo & 48.68 & 79.98 & 88.51 & \ul{97.49} & 76.39 & 90.12 & \ul{95.86} \\
 & Pre. LaSCo w/cap. & \textbf{49.35} & \textbf{80.02} & \textbf{88.75} & 97.47 & \textbf{76.48} & \ul{90.37} & 95.71 \\ \hline
\end{tabular}
}
\end{center}
\caption{Accuracy on CIRR test. set. Note the competitive results of zero-shot model pretrained on \ourDS, w.r.t previous methods trained on CIRR (see \cref{tab:cirr_test}).}
\label{tab:cirr_val}
\end{table}
